Agnostic cosmology in the CAMEL framework

Cosmological parameter estimation is traditionally performed in the Bayesian context. By adopting an "agnostic" statistical point of view, we show the interest of confronting the Bayesian results to a frequentist approach based on profile-likelihoods. To this purpose, we have developed the Cosmological Analysis with a Minuit Exploration of the Likelihood ("CAMEL") software. Written from scratch in pure C++, emphasis was put in building a clean and carefully-designed project where new data and/or cosmological computations can be easily included. CAMEL incorporates the latest cosmological likelihoods and gives access from the very same input file to several estimation methods: (i) A high quality Maximum Likelihood Estimate (a.k.a "best fit") using MINUIT ; (ii) profile likelihoods, (iii) a new implementation of an Adaptive Metropolis MCMC algorithm that relieves the burden of reconstructing the proposal distribution. We present here those various statistical techniques and roll out a full use-case that can then used as a tutorial. We revisit the $\Lambda$CDM parameters determination with the latest Planck data and give results with both methodologies. Furthermore, by comparing the Bayesian and frequentist approaches, we discuss a "likelihood volume effect" that affects the optical reionization depth when analyzing the high multipoles part of the Planck data. The software, used in several Planck data analyzes, is available from http://camel.in2p3.fr. Using it does not require advanced C++ skills.

==> figures/bestprofile_omegab/caption.tex <==
\label{fig:bestprof_omegab}
Construction of the 68\%CL interval by thresholding the interpolated $\omb$ profile-likelihood (in red) at 1.

==> figures/bestprofile_omegab/size.tex <==
height = 700\nwidth = 500

==> figures/camel_alone/caption.tex <==



==> figures/camel_alone/size.tex <==
width=150

==> figures/camel_alone1/caption.tex <==
{}

==> figures/camel_alone1/size.tex <==
width=250

==> figures/camel_alone2/caption.tex <==
{}

==> figures/camel_alone2/size.tex <==
width=200

==> figures/camel_alone3/caption.tex <==
Replace this text with your caption

==> figures/camel_alone3/size.tex <==
width=200

==> figures/camel_transp_rsz/caption.tex <==
  

==> figures/camel_transp_rsz/size.tex <==
width=200

==> figures/coprof_omegab/caption.tex <==
\label{fig:coprof_omegab}
Each plot shows the value of the $\theta_i$ parameter w.r.t to the scanned variable ($\omb$) at the best-fit solutions. We call these curves "co-profiles". They are an indication whether the 2D profile-likelihoods are Gaussian (in which case they should be slopes).

==> figures/coprof_omegab/size.tex <==
width=1000

==> figures/cov/caption.tex <==
\label{fig:cor}
Empirical correlation matrix of the parameters reconstructed from the well-converged chains. The diagonal terms, which are just 1 and were already discussed, are not shown.

==> figures/cov/size.tex <==
height = 700\nwidth = 500

==> figures/gr_MC/caption.tex <==
\label{fig:GR}
Gelman-Rubin test on the 4 chains for the sampled \parfile file. The standard cut is to use samples above $(R-1) \ge 0.03$ and is shown as a dashed line.

==> figures/gr_MC/size.tex <==
width=500

==> figures/histos/caption.tex <==
Replace this text with your caption

==> figures/histos/size.tex <==
height = 700\nwidth = 500

==> figures/histos1/caption.tex <==
\label{fig:histos}

Comparsion of the histograms of each variable for samples above 100000. The result for each chain is shown in different colors.

==> figures/histos1/size.tex <==
width=1000

==> figures/hlpTT_bflike_LCDM_MC/caption.tex <==
\label{fig:post1}
full lines: 1D posterior distributions of MCMC samples obtained by histograming + smoothing the well-converged chain. For clarity the maximum is normalized to 1. We also superimpose in dashed the output of the best-fit values with errors taken from the Hessian matrix. The last 2 parameters are MCMC-derived ones and have thus no associated best-fits.

==> figures/hlpTT_bflike_LCDM_MC/size.tex <==
width=1000

==> figures/hlpTT_bflike_LCDM_MC0/caption.tex <==
\label{fig:trace}
Plots of the values of each variable generated with the MCMC algorithm for one chain using \parfile. The first one displays the $\chi^2$ evolution. The last 2 variables are derived parameters.

==> figures/hlpTT_bflike_LCDM_MC0/size.tex <==
width=1200

==> figures/input_cor/caption.tex <==
\label{fig:Hessian}
Hessian correlation matrix as obtained from the \minuit minimization. It was used as our MCMC proposal.

==> figures/input_cor/size.tex <==
height = 700\nwidth = 500

==> figures/likvspost/caption.tex <==
\label{fig:likvspost}
Reionization optical depth posterior (in red) obtained by sampling, with the AM algorithm, the \planck\ \hiell-only likelihood ({\tt plik}). The corresponding profile likelihood is superimposed in black.

==> figures/likvspost/size.tex <==
height = 700\nwidth = 500

==> figures/marg_vs_lik/caption.tex <==
\label{fig:toy}
A toy example of a 2D likelihood (upper plot) and (bottom plots)the corresponding distributions for the $x_1$ marginalized posterior (in blue) and its profile-likelihood (in red). 

==> figures/marg_vs_lik/size.tex <==
width=300

==> figures/mprof_omega_b/caption.tex <==
\label{fig:mprof_omegab}
\dchi minima reached with different starting points (6) for $\omb$ scanned values. The profile likelihood is obtained as the minimal values for each abcissa point and shown in red. 

==> figures/mprof_omega_b/size.tex <==
height = 700\nwidth = 500

==> figures/pipeline/caption.tex <==
\label{fig:pipeline}
Schematics of the CPE pipeline. From left to right: $\Omega$ denotes the cosmological parameters that feed the Engine which computes some observable(s): $X(\Omega)$. $\nu$ denotes the nuisance parameters of the likelihood (or any external data necessary to its computation). The last 3 vertical boxes show different statistical methods.
Some implementations of engines and likelihoods available in \camel are derived from the base abstract classes.

==> figures/pipeline/size.tex <==
height = 700\nwidth = 500

==> figures/post_vs_hessian/caption.tex <==
\label{fig:cors}
Correlation matrix between all the parameters estimated from the sampled posterior (on the left) and the Hessian matrix (on the right).

==> figures/post_vs_hessian/size.tex <==
width=1000

==> figures/prof_omega_b1/caption.tex <==
\label{fig:prof_omegab1}
A first reconstruction of the omega\_b profile likelihood points using \parfile with one single starting point

==> figures/prof_omega_b1/size.tex <==
height = 700\nwidth = 500

==> figures/prof_vs_mc/caption.tex <==
\label{fig:prof_vs_mc}
The MCMC posterior distributions (in black) as shown previously on Fig. \ref{fig:post1} are compared to the profile-likelihoods (in red , same than those on Fig. \ref{fig:lcdm_prof} but represented here as  $e^{-\dchi/2}$) for the \lcdm\ cosmological parameters using in both cases the same \parfile setup. The dashed lines are here to recall that 68\% level interval are not obtained in the same way: for posteriors the interval is given on the abscissa (as mean $\pm 1 \sigma$), while for profile likelihood the prescription $\dchi=1 \implies \lik/\lik_\textrm{max}= e^{-1/2}$ defines the cut along the ordinate.  Both intervals agree in the Gaussian case.

==> figures/prof_vs_mc/size.tex <==
height = 700\nwidth = 500

==> figures/profile_logA/caption.tex <==
Replace this text with your caption

==> figures/profile_logA/size.tex <==
width=300

==> figures/profile_ns/caption.tex <==
Replace this text with your caption

==> figures/profile_ns/size.tex <==
width=300

==> figures/profile_omega_b/caption.tex <==
Replace this text with your caption

==> figures/profile_omega_b/size.tex <==
height = 700\nwidth = 500

==> figures/profile_omega_cdm/caption.tex <==
Replace this text with your caption

==> figures/profile_omega_cdm/size.tex <==
width=300

==> figures/profile_tau_reio/caption.tex <==
Replace this text with your caption

==> figures/profile_tau_reio/size.tex <==
width=300

==> figures/profile_thetas/caption.tex <==
Replace this text with your caption

==> figures/profile_thetas/size.tex <==
height = 700\nwidth = 500

==> figures/profile_thetas1/caption.tex <==
Replace this text with your caption

==> figures/profile_thetas1/size.tex <==
width=300

==> figures/profs_lcdm/caption.tex <==
\label{fig:lcdm_prof}
Profile-likelihood reconstructed for the 6 \lcdm\ cosmological parameters with the \parfile\ parameter file. The line at 1 gives the 68\% CL region of each parameter.

==> figures/profs_lcdm/size.tex <==
width=1000

==> figures/scan_omb/caption.tex <==
\label{fig:scanomb}

==> figures/scan_omb/size.tex <==
height = 700\nwidth = 500

==> figures/scan_omb1/caption.tex <==

\label{fig:scanomb}
The upper plot shows the $\chi^2$ values obtained from the {\tt ScanParam} program using the \parfile setup, in blue when not specifying any precision file for \class and in red using the hpjul2 one. A smooth fit is superimposed in black. The lower plot shows the residuals in both configurations and reflects the numerical noise of the Boltzmann Engine.




==> figures/scan_omb1/size.tex <==
height = 700\nwidth = 500

==> figures/triangle_test/caption.tex <==
\label{fig:triangle}
"Triangle plot" for the MCMC samples showing the 1D and 2D posterior distributions of the cosmological parameters from the \parfile run. Ellipses show the 68 and 95\% credible intervals.

==> figures/triangle_test/size.tex <==
width=600
